Easy steps towards a sane IT policy in hospitals

We witnessed the low quality of IT solutions in Paris hospitals. The price paid to private companies for these solutions and the cost incurred from their inefficiency constitute a gross and appalling waste of public resources. We propose to bootstrap a change in IT policy by having heads of department hire IT workers ; we give advice to the central decision making body on how to incentivize them. Easily measurable efficiency gains as well as hard-to-quantify positive externalities will follow.

==> bin/cbpaste <==
#!/usr/bin/env python3
# Answer lies in https://groups.google.com/forum/#!topic/comp.os.plan9/WIRK2xFGMVM
# open addr, write ctl, then read addr

import sys
import os
import pyperclip

NAMESPACE = os.getenv('NAMESPACE')
ACME_MNT = NAMESPACE+'/mnt/acme/'

winid = os.getenv('winid')
print(os.getenv('winid'))


with open(ACME_MNT+winid+'/addr', 'a+') as addr:
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('addr=dot\n')
	with open(ACME_MNT+winid+'/data','a+') as data:
                data.write(pyperclip.paste())
	print('wrote "'+pyperclip.paste()+'"')
	


==> bin/cbpaste_ <==
#!/usr/bin/env python3
# Answer lies in https://groups.google.com/forum/#!topic/comp.os.plan9/WIRK2xFGMVM
# open addr, write ctl, then read addr

import sys
import os

print('Hello World')
print(sys.argv)
print(os.getcwd())
winid = os.getenv('winid')
print(os.getenv('winid'))


with open('/tmp/ns.Loulou/mnt/acme/'+winid+'/addr', 'a+') as addr:
	with open('/tmp/ns.Loulou/mnt/acme/'+winid+'/ctl','a') as ctl:
		ctl.write('addr=dot\n')
	addr.write('.-+')
	print('addr read : '+addr.read())
	
with open('/tmp/ns.Loulou/mnt/acme/'+winid+'/xdata','r') as data:
	print(data.read())
	


==> bin/lenv <==
#!/usr/bin/env python3
"""Insert a LaTeX env at point"""
# Answer lies in https://groups.google.com/forum/#!topic/comp.os.plan9/WIRK2xFGMVM
# open addr, write ctl, then read addr

import sys
import os
import re

NAMESPACE = os.getenv('NAMESPACE')
ACME_MNT = NAMESPACE+'/mnt/acme/'

try:
	env = sys.argv[1]
except IndexError:
	env = 'itemize' #Default env
try:
	winid = sys.argv[2]
except IndexError:
	winid = os.getenv('winid')


to_be_written = "\\begin{{{env}}}\n\n\\end{{{env}}}".format(env=env)

with open(ACME_MNT+winid+'/addr', 'a+') as addr:
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('addr=dot\n')
	
with open(ACME_MNT+winid+'/data','a') as data:
	data.write(to_be_written)

with open(ACME_MNT+winid+'/addr', 'a+') as addr:
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('addr=dot\n')
	addr.write('.-')
with open(ACME_MNT+winid+'/ctl','a') as ctl:
	ctl.write('dot=addr\n')
	

#print(to_be_written)


==> bin/lh+ <==
#!/usr/bin/env python3
"""Script to use with plan9port's acme : increase rank of LaTeX heading at point"""
# Answer lies in https://groups.google.com/forum/#!topic/comp.os.plan9/WIRK2xFGMVM
# open addr, write ctl, then read addr

import sys
import os
import re

NAMESPACE = os.getenv('NAMESPACE')
ACME_MNT = NAMESPACE+'/mnt/acme/'


try:
	winid = sys.argv[1]
except IndexError:
	winid = os.getenv('winid')


with open(ACME_MNT+winid+'/addr', 'a+') as addr:
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('addr=dot\n')
	addr.write('.-+')
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('dot=addr\n')
	
with open(ACME_MNT+winid+'/xdata','r') as data:
	line_at_dot = data.read()

heading_list = [ 'paragraph', 'subsubsection', 'subsection', 'section', 'chapter']

heading_regex = r'\\('+'|'.join(heading_list)+')\{([^\n]*)\}'

rem = re.match(heading_regex, line_at_dot.strip())
if rem:
	header = rem.group(1)
	contents = rem.group(2)
	new_header = heading_list[heading_list.index(header)+1]
else:
	new_header = 'paragraph'
	contents = line_at_dot.strip()

to_be_written = "\\"+new_header+r'{'+contents+"}\n"


with open(ACME_MNT+winid+'/addr', 'a+') as addr:
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('addr=dot\n')
	addr.write('.-+')
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('dot=addr\n')
with open(ACME_MNT+winid+'/data','a+') as data:
	data.write(to_be_written)
with open(ACME_MNT+winid+'/addr', 'a+') as addr:
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('addr=dot\n')
	addr.write('-')
with open(ACME_MNT+winid+'/ctl','a+') as ctl:
	ctl.write('dot=addr\n')	

#with open(ACME_MNT+winid+'/addr', 'a+') as addr:
#	with open(ACME_MNT+winid+'/ctl','a') as ctl:
#		ctl.write('addr=dot\n')
#	addr.write('.-')
#with open(ACME_MNT+winid+'/ctl','a') as ctl:
#	ctl.write('dot=addr\n')
	

#print(to_be_written)


==> bin/lh- <==
#!/usr/bin/env python3
"""Script to use with plan9port's acme : decrease rank of LaTeX heading at point"""
# Answer lies in https://groups.google.com/forum/#!topic/comp.os.plan9/WIRK2xFGMVM
# open addr, write ctl, then read addr

import sys
import os
import re

NAMESPACE = os.getenv('NAMESPACE')
ACME_MNT = NAMESPACE+'/mnt/acme/'

try:
	winid = sys.argv[1]
except IndexError:
	winid = os.getenv('winid')


with open(ACME_MNT+winid+'/addr', 'a+') as addr:
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('addr=dot\n')
	addr.write('.-+')
	
with open(ACME_MNT+winid+'/xdata','r') as data:
	line_at_dot = data.read()

heading_list = [ 'paragraph', 'subsubsection', 'subsection', 'section', 'chapter']

heading_regex = r'\\('+'|'.join(heading_list)+')\{([^\n]*)\}'

rem = re.match(heading_regex, line_at_dot.strip())
if rem:
	header = rem.group(1)
	contents = rem.group(2)
	new_header = heading_list[heading_list.index(header)-1]
else:
	new_header = 'paragraph'
	contents = line_at_dot.strip()

to_be_written = "\\"+new_header+r'{'+contents+"}\n"

with open(ACME_MNT+winid+'/addr', 'a+') as addr:
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('addr=dot\n')
	addr.write('.-+')
	
with open(ACME_MNT+winid+'/data','a') as data:
	data.write(to_be_written)
	
with open(ACME_MNT+winid+'/addr', 'a+') as addr:
	with open(ACME_MNT+winid+'/ctl','a') as ctl:
		ctl.write('addr=dot\n')
	addr.write('.-')
with open(ACME_MNT+winid+'/ctl','a') as ctl:
	ctl.write('dot=addr\n')
	

#print(to_be_written)

